FLARE: Robot Learning with Implicit World Modeling

We introduce $\textbf{F}$uture $\textbf{LA}$tent $\textbf{RE}$presentation Alignment ($\textbf{FLARE}$), a novel framework that integrates predictive latent world modeling into robot policy learning. By aligning features from a diffusion transformer with latent embeddings of future observations, $\textbf{FLARE}$ enables a diffusion transformer policy to anticipate latent representations of future observations, allowing it to reason about long-term consequences while generating actions. Remarkably lightweight, $\textbf{FLARE}$ requires only minimal architectural modifications -- adding a few tokens to standard vision-language-action (VLA) models -- yet delivers substantial performance gains. Across two challenging multitask simulation imitation learning benchmarks spanning single-arm and humanoid tabletop manipulation, $\textbf{FLARE}$ achieves state-of-the-art performance, outperforming prior policy learning baselines by up to 26%. Moreover, $\textbf{FLARE}$ unlocks the ability to co-train with human egocentric video demonstrations without action labels, significantly boosting policy generalization to a novel object with unseen geometry with as few as a single robot demonstration. Our results establish $\textbf{FLARE}$ as a general and scalable approach for combining implicit world modeling with high-frequency robotic control.

==> figures/raw/24p_results.tex <==
% \begin{table*}[htbp]
% \centering
% \scriptsize
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Task Name} & \textbf{FLARE (\%)} & \textbf{FLARE w/. Policy Only (\%)} & \textbf{UWM (\%)} & \textbf{Groot-N1 (\%)} & \textbf{Diffusion Policy (\%)} \\
% \midrule
% CloseDoubleDoor & 88.89 & 85.71 & 87.25 & 82.35 & 84.17 \\
% CloseDrawer & 100.00 & 100.00 & 99.02 & 99.02 & 96.67 \\
% CloseSingleDoor & 98.15 & 96.43 & 94.12 & 89.22 & 87.50 \\
% CoffeePressButton & 96.30 & 89.29 & 76.47 & 92.16 & 87.50 \\
% CoffeeServeMug & 70.37 & 67.86 & 64.71 & 71.57 & 69.17 \\
% CoffeeSetupMug & 53.70 & 41.07 & 27.45 & 32.35 & 34.17 \\
% OpenDoubleDoor & 48.15 & 14.29 & 28.43 & 18.63 & 21.67 \\
% OpenDrawer & 94.44 & 80.36 & 82.35 & 82.35 & 75.83 \\
% OpenSingleDoor & 77.78 & 78.57 & 83.33 & 60.78 & 72.50 \\
% PnPCabToCounter & 55.56 & 35.71 & 23.53 & 23.53 & 8.33 \\
% PnPCounterToCab & 42.59 & 51.79 & 40.20 & 49.02 & 26.67 \\
% PnPCounterToMicrowave & 31.48 & 23.21 & 25.49 & 28.43 & 14.17 \\
% PnPCounterToSink & 59.26 & 35.71 & 28.43 & 40.20 & 30.00 \\
% PnPCounterToStove & 68.52 & 42.86 & 46.08 & 37.25 & 31.67 \\
% PnPMicrowaveToCounter & 51.85 & 51.79 & 27.45 & 33.33 & 22.50 \\
% PnPSinkToCounter & 59.26 & 57.14 & 37.25 & 58.82 & 42.50 \\
% PnPStoveToCounter & 66.67 & 66.07 & 50.98 & 61.76 & 38.33 \\
% TurnOffMicrowave & 96.30 & 94.64 & 91.18 & 91.18 & 60.00 \\
% TurnOffSinkFaucet & 94.44 & 92.86 & 93.14 & 89.22 & 83.33 \\
% TurnOffStove & 25.93 & 30.36 & 23.53 & 18.63 & 39.17 \\
% TurnOnMicrowave & 88.89 & 83.93 & 83.33 & 72.55 & 70.83 \\
% TurnOnSinkFaucet & 79.63 & 71.43 & 81.37 & 78.43 & 78.33 \\
% TurnOnStove & 68.52 & 37.50 & 78.43 & 69.61 & 27.50 \\
% TurnSinkSpout & 66.67 & 57.14 & 85.29 & 73.53 & 37.50 \\
% \bottomrule
% \end{tabular}
% \caption{Per-task success rates across different methods on RoboCasa-PandaOmron tasks (all numbers in percentages).}
% \label{tab:robocasa_per_task_results}
% \end{table*}
